Is Mapping Necessary for Realistic PointGoal Navigation?

Can an autonomous agent navigate in a new environment without building an explicit map? For the task of PointGoal navigation ('Go to $\Delta x$, $\Delta y$') under idealized settings (no RGB-D and actuation noise, perfect GPS+Compass), the answer is a clear 'yes' - map-less neural models composed of task-agnostic components (CNNs and RNNs) trained with large-scale reinforcement learning achieve 100% Success on a standard dataset (Gibson). However, for PointNav in a realistic setting (RGB-D and actuation noise, no GPS+Compass), this is an open question; one we tackle in this paper. The strongest published result for this task is 71.7% Success. First, we identify the main (perhaps, only) cause of the drop in performance: the absence of GPS+Compass. An agent with perfect GPS+Compass faced with RGB-D sensing and actuation noise achieves 99.8% Success (Gibson-v2 val). This suggests that (to paraphrase a meme) robust visual odometry is all we need for realistic PointNav; if we can achieve that, we can ignore the sensing and actuation noise. With that as our operating hypothesis, we scale the dataset and model size, and develop human-annotation-free data-augmentation techniques to train models for visual odometry. We advance the state of art on the Habitat Realistic PointNav Challenge from 71% to 94% Success (+23, 31% relative) and 53% to 74% SPL (+21, 40% relative). While our approach does not saturate or 'solve' this dataset, this strong improvement combined with promising zero-shot sim2real transfer (to a LoCoBot) provides evidence consistent with the hypothesis that explicit mapping may not be necessary for navigation, even in a realistic setting.

==> sections/old/1_introduction.tex <==
\section{Introduction}
\begin{figure}[ht!]
    \begin{center}
        \includegraphics[width=1\linewidth]{assets/approach_schema_v2.png}
\end{center}
\caption{Agent architecture for Realistic PointGoal navigation. It consists of two components: RL navigation policy and visual odometry module. Where  $g_{t-1}$ - goal coordinates (wrt. current pose), $a_t$ - action to take, $h_{t-1}$ and $h_t$ - hidden states. Predicted pose change is subtracted from the goal location and the result is fed into policy as a new goal location. The initial goal location estimate is equal to ground truth goal location.} 
\label{fig:policy_vo}
\end{figure}
With advances in science and engineering, technologies that were expensive and used only by large corporations or government departments became cheaper and move from laboratories to our houses. 

Even though current progress in autonomous robotics is distant from how it is described in science fiction, the study of intelligent systems with a physical or virtual embodiment (Embodied AI) is already being used in many different applications. In particular, the latest versions of the Roomba \footnote{Roomba is a series of autonomous robotic vacuum cleaners sold by iRobot.} robot vacuum cleaner use suite of sensors and visual localization system to learn and remember where objects are in a room, so that the robot knows exactly where it is, where it has been and where it needs to go next.  But Embodied AI tasks extend far beyond exploration \footnote{Exploration is an Embodied AI task where the objective is to maximize the coverage in a fixed time budget.}, for instance, gripping and moving objects to specified locations or natural language instructions following. 
The potential benefits of AI assistants of the future range from conveniences, such as asking a robot to get a set of keys from the kitchen to helping the visually impaired navigate unfamiliar environments or perform complex tasks in dangerous or difficult situations. % 

Growing number of scientific papers published and competitions/workshops held at top Computer Vision / Machine Learning conferences \cite{wijmans2020dd,chaplot2020learning,ramakrishnan2020occupancy,datta2020integrating} indicate the interest in the Embodied AI domain. The important question that is raised in recent publications is the ability of intelligent system to efficiently navigate in real-world environments \cite{kadian2019are,datta2020integrating}. Research community has introduced wide range of navigation tasks \cite{anderson2018on} so far. Proposed tasks can be distinguished by the type of goal the agent should navigate to:  PointGoal - specific location, ObjectGoal - given object class, AreaGoal - area of a specified category.

In PointGoal navigation (PointNav) agent is initialized in previously unseen environment and it's task is to reach the goal (stop within success zone that is equal to 2 $\times$ agent radius) that is specified relative to start location. The action space is discrete and consists of four types of actions: STOP - finish navigation episode, MOVE\_FORWARD - move $0.25m$ forward; TURN\_LEFT - turn $30^{\degree}$ left, TURN\_RIGHT - turn $30^{\degree}$ right.

In PoitNav v1 setting the agent has an access to precise localization via so called GPS+Compass, it's RGB-D input is noiseless and actuation is deterministic (i.e. the same sequence of actions lead to the same location in the environment; agent moves exactly $0.25m$ and rotates exactly $30^{\degree}$) and it could even ‘slide’ along the walls. This setting is considered solved by approach proposed in \cite{wijmans2020dd} that is successful in $99.7\%$ of episodes and follows near-perfect path reaching $97$ $SPL$. However, due to unrealistic task specification such an impressive scores in simulation do not persist after physical deployment. \cite{kadian2019are} show that in PoitNav v1 setting correlation between scores nav-agents got in simulation and reality is quite low (i.e. low $sim2real$ score). It means that high score/progress in simulation may not generalize to real robotic testbeds.  

As the community's main goal is, actually, having robots operating well after physical deployment and inspired by findings in \cite{kadian2019are}, new PoitNav v2 ("realistic") setting was introduced. Specifically, the following changes were made: 
\begin{itemize}
    \item no precise localization via GPS+Compass (agent needs to perform RGBD-based online localization)
    \item noisy actuation and sensing (noisy RGB-D; agent may experience rotation and translation noise both while rotating and moving forward; identical action sequences can lead to vastly different final locations)
    \item  ‘sliding’ along the walls is disabled
    \item agent’s camera’s tilt angle is set to $-20^{\degree}$ (in PointNav~v1 tilt angle is $0^{\degree}$)
\end{itemize}

State-of-the-art (SOTA) approaches in noiseless setting turned out to perform poorly without precise localization and under noisy conditions. So solution of realistic PointGoal navigation problem – odometry for robot navigation – is another milestone towards building truly autonomous robots, be it C3PO, Marvin or Terminator. 

Straightforward modification of PoitNav v1 SOTA approach where the ground truth localization signal is replaced with it's estimate from visual odometry model (sometimes referred to as pose estimator; module that computes relative pose change given two consecutive RGB-D frames) show competitive results in  PoitNav v2. But despite extensive research PoitNav v2  continues to be an open frontier for Embodied AI research. According to the Habitat Challenge 2020 \footnote{Online benchmark: \href{https://aihabitat.org/challenge/2020}{https://aihabitat.org/challenge/2020}} PointGoal navigation benchmark, operating in the noisy environments SOTA approaches can reach the destination in 71.7\% of cases with 0.525 SPL score (28\% Success and 0.444 SPL gap from PoitNav v1). 

So in this paper we try to answer the questions that naturally arise:
\begin{itemize}
    \item can the PoitNav v1 and PoitNav v2 Success and SPL gap be closed?
    \item is the visual odometry module is all you need to close the gap?
    \item will the PoitNav v2 agent that does fully visual/perceptual navigation transfer from simulation to reality?
\end{itemize}

% increasing confidence that in-simulation comparisons will translate to deployed systems in reality.



% Since launched in the house robot has to avoid/step over stairs, deal with obstacles/clutter and different types of surface properties and lightning conditions. The focus is on increased realism i.e. experimental setups are designed to match the real world environment as close as possible \cite{kadian2019are}. That is achieved by using photorealistic 3D scans of real buildings in simulation and incorporating actuation and sensing noise models.

% Among the different sensor modalities, cameras are cheap and provide rich information of the environment that allows for robust and accurate place recognition. Moreover, compass and GPS data can be too noisy or simply unavailable in indoor spaces. Therefore, visual navigation solutions where the main sensor is a RGB-D camera are of major interest nowadays.
% To answer the aforementioned questions we ...
The main contributions of our work are:
\begin{itemize}
    \item we estimate that due to actuation noise actual PointNav~v2 max is $84$ $SPL$, not $99$ $SPL$ as in PointNav~v1. Consequently, PointNav~v2 can be considered solved when $84$ $SPL$ and $100\%$ Success is reached.
    \item we present simple yet efficient regularization techniques (implemented as train/test augmentations) and optimized VO module architecture that gives only 4 points $SPL$ and Success hit to GT nav-policy on Gibson~v2 validation scenes (even without fine-tuning!). We perform an extensive ablation study of proposed modifications and show their influence on the downstream navigation metrics of map-free deep learned agents (action embedding: +8 Success, + 6 SPL; train/test Augmentations: +5 Success, + 4 SPL; larger dataset (0.5M  $\rightarrow$ 1.5M): +8 Success + 6 SPL; more powerful encoder (ResNet18$\rightarrow$ResNet50): +3 Success + 3SPL). We report navigation metrics on Gibson~v2/MP3D~v2/Habitat Challenge 2021 test-standard datasets.
    \item nav-agent equipped with out VO sets new SOTA on Habitat Challenge 2021 PointNav v2 online benchmark scoring 94 $Success$ and 74 $SPL$ (reducing the gap to potential maximum to 6 $Success$ points and 10 $SPL$ points) 
    \item run small-size experiments to show Sim2real transfer 
    \item to support the community interest and push Embodied AI research forward we opensource our code and model checkpoints (with distributed VO training pipeline and distributed VO dataset generation code that significantly speed ups research process when working with large datasets).  
    \item we share our ideas of future work
    
\end{itemize}



% In this work we focus on closing the SPL/Success gap between agent with access to ground-truth localization and agent estimating it's egomotion from RGBD camera images.
% We propose train/test-time augmentations that increase visual odometry noise robustness.
% And show that PointNav v2 setting is totally learnable as PointNav v1.

% Novelty: 
% \begin{itemize}
%     \item PointNavV2 is totally learnable
%     \item VO module != VO model
%     \item Distributed VO training pipeline (engineering)
%     \item ... 
% \end{itemize}



% \href{https://www.springwise.com/tech-explained-embodied-ai/}{here}. 

% \textcolor{red}{Explain sim to real predictivity?}. 

% the developed approaches can be transferred to other navigation tasks. 

% TODO: illustrate Embodied AI benchmarks/challenges/workshops (Partners and embodied AI challenges at CVPR 2021) \href{https://ai.facebook.com/blog/2021-habitat-challenge-launches-to-advance-embodied-ai-research/}{2021 Habitat Challenge launches to advance embodied AI research}

% TODO: add a few words to transition to navigation more smoothly

% \href{https://ai.facebook.com/blog/2021-habitat-challenge-launches-to-advance-embodied-ai-research/?__cft__[0]=AZW9nT1vjmjUj3Z68uwSqtFXM7s9o7EPacWiUu_lzyBifOSVPWtB4Y90td2mZ4EIDQoyj9JHUfcnHFErdn8yGYdyk4YL35v0PR85LC7HqALk4FHsLofHzlB83uiWyAHeNeXJ2ZC-QZ6EWAyr9CG_42jl}{source}.

% \textcolor{red}{The potential benefits of this work range beyond conveniences, such as asking a robot to get a set of keys from the kitchen or a laptop from a desk upstairs. Embodied AI can also, for example, help the visually impaired navigate unfamiliar environments or perform difficult tasks in dangerous or difficult situations.}

% TODO: explain Roomba is a series of autonomous robotic vacuum cleaners sold by iRobot
% TODO: explain "exploration"

% As a result, the study of intelligent systems with a physical or virtual embodiment (Embodied AI) is getting more and more attention from the research community nowadays. 
% \textcolor{red}{Explain Embodied AI a little bit more: Perception, long term planning, episodic memory interaction with the world}.

==> sections/old/old_tables.tex <==
\begin{table*}[h!]
\begin{center}

\begin{tabular}{l|c|c|c|c|cccc|cc|cccc}
\hline\hline
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{Dataset} &
\multicolumn{1}{c}{\multirow{2}{*}{Encoder}} &
\multicolumn{1}{c}{\multirow{1}{*}{\#params}} &
\multicolumn{1}{c}{\multirow{2}{*}{Epoch}} &
\multicolumn{4}{c}{Train time} &
\multicolumn{2}{c}{Test time} &
\multicolumn{4}{c}{Navigation metrics (${e}^{-2}$)} 
\\
\multicolumn{1}{l}{} &
\multicolumn{1}{c}{size(M)} &                               
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{(M)} & 
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{1FC} &
\multicolumn{1}{c}{2FC} &
\multicolumn{1}{c}{Flip} &
\multicolumn{1}{c}{Swap} &
\multicolumn{1}{c}{Flip} &
\multicolumn{1}{c}{Swap} &
\multicolumn{1}{c}{$S$} &
\multicolumn{1}{c}{$SPL$} &
\multicolumn{1}{c}{$SoftSPL$} &
\multicolumn{1}{c}{$d_G$} 
\\ 
\hline\hline
1                   & 0.5 & resnet18 &  4.2                  & 50                  &            &            &            &            &            &            & 64 & 52 & 73 & 58 \\ \hline
2                   & 0.5 & resnet18 &  4.2                 & 43                  & \checkmark &            &            &            &            &            & 71 & 57 & 73 & 44 \\ \hline
3                   & 0.5 & resnet18 &  4.2                 & 44                  & \checkmark & \checkmark &            &            &            &            & 72 & 58 & 73 & 43 \\ \hline
\multirow{2}{*}{4}  & \multirow{2}{*}{0.5} & \multirow{2}{*}{resnet18} & \multirow{2}{*}{4.2 } & \multirow{2}{*}{48} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & & \multirow{2}{*}{\checkmark} &  & & 70 & 56 & 73 & 51 \\
                    & & &                     &                     &                             &                             & & &            & \checkmark & 71 & 57 & 73 & 54 \\ \hline
\multirow{2}{*}{5}  & \multirow{2}{*}{0.5} & \multirow{2}{*}{resnet18} & \multirow{2}{*}{4.2} & \multirow{2}{*}{50} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & & & & 74 & 59 & 74 & 40 \\
                    & & &                     &                     &                             &                             & & & \checkmark & & 76 & 61 & 74 & 37 \\ \hline
\multirow{4}{*}{6}  & \multirow{4}{*}{0.5} &  \multirow{4}{*}{resnet18} &  \multirow{4}{*}{4.2} & \multirow{4}{*}{50} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\checkmark} & \multirow{4}{*}{\checkmark} & & & 74 & 59 & 73 & 45 \\
                    & & &                      &                     & & & & &            & \checkmark & 76 & 60 & 74 & 40\\ 
                    & & &                     &                     & & & & & \checkmark &            & 76 & 61 & 73 & 39 \\
                    & & &                     &                     & & & & & \checkmark & \checkmark & 77 & 62 & 74 & 37 \\ \hline
7                   & 1.5 & resnet18 &  4.2                  & 48                  & \checkmark & \checkmark &            &            &            &            & 77 & 62 & 74 & 38 \\ \hline
8                   & 1.5 & resnet18 &  4.2                 & 50                  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 85 & 68 & 75 & 32 \\ \hline
9                   & 1.5 & resnet50 &  7.6                 & 48                  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 88 & 71 & 76 & 27 \\
\hline\hline
\end{tabular}
\end{center}
\caption{Evaluation on the Gibson v2 4+ validation split.
Results are reported as an average of four evaluations with different seeds. Navigation metrics: $S$, $SPL$, $SoftSPL$ and $d_G$ (distance to goal) are subject to ${e}^{-2}$ multiplication. Tick in a column indicate whether a particular option is turned on. For instance, in experiments corresponding to row 5 the ResNet-18 is used as VO encoder, action embedding is concatenated to 1-st fully connected and 2-nd fully connected layer, flip augmentation is turned on during training; navigation metrics are reported with flip augmentation on/off during evaluation.}
\label{table:nav_metrics}
\end{table*}



\begin{table*}
\begin{center}

\begin{tabular}{lccccccccccccc}
\toprule
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{Dataset} &
\multicolumn{1}{c}{\multirow{2}{*}{Encoder}} &
\multicolumn{1}{c}{\multirow{1}{*}{\#params}} &
\multicolumn{4}{c}{Train time} &
\multicolumn{2}{c}{Test time} &
\multicolumn{4}{c}{Navigation metrics ($\times10^2$)} 
\\
\multicolumn{1}{l}{} &
\multicolumn{1}{c}{size(M)} &                               
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{(M)} & 
\multicolumn{1}{c}{1FC} &
\multicolumn{1}{c}{2FC} &
\multicolumn{1}{c}{Flip} &
\multicolumn{1}{c}{Swap} &
\multicolumn{1}{c}{Flip} &
\multicolumn{1}{c}{Swap} &
\multicolumn{1}{c}{Success} &
\multicolumn{1}{c}{SPL} &
\multicolumn{1}{c}{SoftSPL} &
\multicolumn{1}{c}{$\text{d}_\text{G}$} 
\\ 
\midrule
1                   & 0.5 & ResNet18 &  4.2                                    &            &            &            &            &            &            & 64 & 52 & 73 & 58 \\ 
2                   & &  &                                & \checkmark &            &            &            &            &            & 71 & 57 & 73 & 44 \\ 
3                   & &  &                            & \checkmark & \checkmark &            &            &            &            & 72 & 58 & 73 & 43 \\ \midrule
4 &  &  &  & \checkmark & \checkmark & & \checkmark &  & 
& 70 & 56 & 73 & 51 \\
5 &  &  &  & \checkmark & \checkmark & & \checkmark &  & \checkmark
& 71 & 57 & 73 & 54 \\ \midrule

6 &  &  & & \checkmark & \checkmark & \checkmark & & & & 
74 & 59 & 74 & 40 \\
7 &  &  & & \checkmark & \checkmark & \checkmark & & \checkmark & & 
76 & 61 & 74 & 37 \\ \midrule

8 &  &  & & \checkmark & \checkmark & \checkmark & \checkmark & & & 
 74 & 59 & 73 & 45 \\
9 &  &  & & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & 
 76 & 60 & 74 & 40\\ 
10 &  &  & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & 
 76 & 61 & 73 & 39 \\
11 &  &  & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 
 77 & 62 & 74 & 37 \\ 
 \midrule
12  & 1.5 & ResNet18 & 4.2 & \checkmark & \checkmark &            &            &            &            
& 77 & 62 & 74 & 38 \\ 
13 & & & &   \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 85 & 68 & 75 & 32 \\ \midrule
14 & 1.5 & ResNet50 &  7.6 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 88 & 71 & 76 & 27 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Evaluation on the Gibson v2 4+ validation split.
Results are reported as an average of four evaluations with different seeds. Navigation metrics: $S$, $SPL$, $SoftSPL$ and $d_G$ (distance to goal) are subject to ${e}^{-2}$ multiplication. Tick in a column indicate whether a particular option is turned on. For instance, in experiments corresponding to row 5 the ResNet-18 is used as VO encoder, action embedding is concatenated to 1-st fully connected and 2-nd fully connected layer, flip augmentation is turned on during training; navigation metrics are reported with flip augmentation on/off during evaluation.}
\label{table:nav_metrics}
\end{table*}
